Dissecting Causal Biases

Accurately measuring discrimination in machine learning-based automated decision systems is required to address the vital issue of fairness between subpopulations and/or individuals. Any bias in measuring discrimination can lead to either amplification or underestimation of the true value of discrimination. This paper focuses on a class of bias originating in the way training data is generated and/or collected. We call such class causal biases and use tools from the field of causality to formally define and analyze such biases. Four sources of bias are considered, namely, confounding, selection, measurement, and interaction. The main contribution of this paper is to provide, for each source of bias, a closed-form expression in terms of the model parameters. This makes it possible to analyze the behavior of each source of bias, in particular, in which cases they are absent and in which other cases they are maximized. We hope that the provided characterizations help the community better understand the sources of bias in machine learning applications.

==> tex-input-files/text-confoundingBias.tex <==


Confounding bias occurs when both the sensitive variable and the outcome have a common cause, the counfounder variable. Consequently, the mechanism of selecting samples from the two groups (protected and privileged) is not independent of the outcome. This creates a bias when measuring the causal effect of the sensitive attribute on the outcome. 


% \begin{figure}[h]
% 	\centering
% 	{\includegraphics[scale=0.6]{./figures/simpleConfounder.pdf}}
% 	\caption{Simple confounding structure}
% 	\label{fig:simpleConf}
% \end{figure}

% \begin{figure*}[htp!]  
% \centering 
%   \begin{subfigure}[t]{}
%   {\includegraphics[scale=0.6]{./figures/simpleConfounder.pdf}}
% 	\caption{}
% 	\label{fig:simpleConfa}
%  \end{subfigure}
%  \hspace{0.05\linewidth}
%  \begin{subfigure}[t]{}
%   {\includegraphics[scale=0.6]{./figures/simpleConfounderLinear.pdf}}
% 	\caption{}
% 	\label{fig:simpleConfb}
%  \end{subfigure}
%  \caption{Simple confounding structure}
%  \end{figure*}
 






%\subsection{Binary Model Case}

For a concise notation, let $y_1$ and $y_0$ denote the propositions $Y=1$ and $Y=0$, respectively, and the same for the variables $A$ and $Z$. For instance, $\pr(Y=1|A=0)$ is written simply as $\pr(y_1|a_0)$. 





\begin{theorem} \label{th:confBin}
Assuming $A$, $Y$, and $Z$ binary variables and that $\pr(a_0) = \pr(a_1) = \frac{1}{2}$\footnote{A result without this assumption can be found in the supplementary material.}, the difference in discrimination due to confounding is equal to:
\begin{align}
ConfBias(Y,A) &= (1- \pr(z_0|a_0) - \pr(z_1))(\alpha -\beta +\gamma -\delta).\label{eq:th:confBin}
\end{align}
%where $\alpha, \beta, \gamma, \delta$ denote, respectively, 
%$\pr(y_1|a_0,z_0), \pr(y_1|a_0,z_1), \pr(y_1|a_1,z_0),\pr(y_1|a_1,z_1)$.
% \end{itemize}
%  where:
% \begin{align}
% % % \tau &= P(a_0|z_0) \nonumber \\
% % % \epsilon &= P(z_0) \nonumber \\
%  \alpha &= \pr(y_1|a_0,z_0) \nonumber \\
%  \beta &= \pr(y_1|a_0,z_1) \nonumber \\
%  \gamma &= \pr(y_1|a_1,z_0) \nonumber \\
%  \delta &= \pr(y_1|a_1,z_1) \nonumber 
%  \end{align}   
\end{theorem}





%\subsection{Linear Model Case}

% \begin{figure}[h]
% 	\centering
% 	{\includegraphics[scale=0.6]{./figures/simpleConfounderLinear.pdf}}
% 	\caption{Confounding structure in linear model}
% 	\label{fig:simpleConfLin}
% \end{figure}

\begin{theorem}
\label{th:confLin}
Let $A$, $Y$, and $Z$ variables with linear regressions coefficients as in Figure~\ref{fig:simpleConfLin} which represents the basic confounding structure. The confounding bias can be expressed in terms of covariances of pairs of variables as follows:
\begin{equation}
\confBias(Y,A) =  \frac{\sigma_{za}\sigma_{yz} - \frac{\sigma_{ya}}{\sigma_a^2}\sigma_{za}^2}{\sigma_a^2\sigma_z^2 - \sigma_{za}^2} \label{eq:confLin1}
\end{equation}
where $\sigma_x^2$ denotes the variance of $X$ and $\sigma_{xy}$ denotes the covariance of $X$ and $Y$.

Confounding bias can also be expressed in terms of the linear regression coefficients as follows:
\begin{equation}
\confBias(Y,A) = \frac{{\sigma_z}^2}{{\sigma_a}^2} \beta \gamma \label{eq:confBiasLin}
\end{equation}
\end{theorem}




\begin{corollary}
\label{cor:confLin}
For standardized variables\footnote{Variables normalized to have a mean $0$ and standard deviation $1$.} $A$, $Y$, and $Z$, confounding bias can be expressed in terms of covariances as:
\begin{equation}
\confBias(Y,A) =  \frac{\sigma_{za}\sigma_{yz} - \sigma_{ya}\sigma_{za}^2}{1 - \sigma_{za}^2} \label{eq:confLin3}
\end{equation}
And in terms of regression coefficient, simply as (~\cite{pearl2013linear}):
\begin{equation} 
\confBias(Y,A) = \beta \gamma \label{eq:confLin4}
\end{equation}
\end{corollary}
Equations~(\ref{eq:confLin3}) and~(\ref{eq:confLin4}) can be obtained from Equations~(\ref{eq:confLin1}) and~(\ref{eq:confBiasLin}) as $\sigma_z = \sigma_a = 1$.

We provide in the supplementary material (Appendix~\ref{ap:twoConf}) the closed-form expression of confounding bias in presence of two (or several confounders) in the linear case.

%\subsection{Linear case with two confounders}



\noindent
\begin{figure}
\begin{minipage}{0.22\linewidth}
\centering
		{\includegraphics[scale=0.5]{./figures/simpleConfounderLinear.pdf}}
	\caption{Confounding structure in linear model}
	\label{fig:simpleConfLin}
\end{minipage}
\hspace{0.3cm}
\begin{minipage}{0.22\linewidth}
\centering
  \includegraphics[scale=0.5]{./figures/simpleColliderLinear.pdf}
	\caption{Simple collider structure}
	\label{fig:simpleColl}
 \end{minipage}
 \hspace{0.3cm}
\begin{minipage}{0.22\linewidth}
\centering
  \includegraphics[scale=0.5]{./figures/measurementBiasLin.pdf}
	\caption{Simple measurement bias structure}
	\label{fig:measBias}
\end{minipage}
\hspace{0.3cm}
\begin{minipage}{0.22\linewidth}
\centering
    \includegraphics[scale=0.5]{figures/Interaction.pdf}
    \caption{Interaction Bias, where $A$ and $B$ are sensitive variables and $Y$ is an outcome.}
    \label{fig:interaction}
\end{minipage}
\end{figure}




% \begin{figure}
% \begin{sufigure}{0.22\linewidth}
% \centering

% 		{\includegraphics[scale=0.5]{./figures/simpleConfounderLinear.pdf}}
% 	\caption{Confounding structure in linear model}
% 	\label{fig:simpleConfLin}

% \end{sufigure}

% \begin{sufigure}{0.22\linewidth}
% \centering
%   \includegraphics[scale=0.5]{./figures/simpleColliderLinear.pdf}
% 	\caption{Simple collider structure}
% 	\label{fig:simpleColl}
 
% \end{sufigure}

% \begin{sufigure}{0.22\linewidth}
% \centering
%   \includegraphics[scale=0.5]{./figures/measurementBiasLin.pdf}
% 	\caption{Simple measurement bias structure}
% 	\label{fig:measBias}

% \end{sufigure}
% \begin{sufigure}{0.22\linewidth}
% \centering
%     \includegraphics[scale=0.5]{figures/Interaction.pdf}
%     \caption{Interaction Bias, where $A$ and $B$ are sensitive variables and $Y$ is an outcome.}
%     \label{fig:interaction}

% \end{sufigure}
% \caption{tt}
% \end{figure}


% \begin{figure}
% \centering
% \begin{subfigure}{.24\textwidth}
%   \centering
%   \includegraphics[width=.4\linewidth]{image1}
%   \caption{A subfigure}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.4\linewidth]{image1}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{A figure with two subfigures}
% \label{fig:test}
% \end{figure}

% \noindent
% \begin{figure}
% \begin{minipage}{0.24\linewidth}
% \begin{figure}
% 		{\includegraphics[scale=0.2]{./figures/simpleConfounderLinear.pdf}}
% 	\caption{Confounding structure in linear model}
% 	\label{fig:simpleConfLin}
% \end{figure}
% \end{minipage}
% \begin{minipage}{0.24\linewidth}
%  \begin{figure} 
%   \includegraphics[scale=0.2]{./figures/simpleColliderLinear.pdf}
% 	\caption{Simple collider structure}
% 	\label{fig:simpleColl}
%  \end{figure}
% \end{minipage}
% \begin{minipage}{0.24\linewidth}
% \begin{figure}
%   \includegraphics[scale=0.2]{./figures/measurementBiasLin.pdf}
% 	\caption{Simple measurement bias structure}
% 	\label{fig:measBias}
% \end{figure}
% \end{minipage}
% \begin{minipage}{0.24\linewidth}
% \begin{figure}
%     \includegraphics[scale=0.2]{figures/Interaction.pdf}
%     \caption{Interaction Bias, where $A$ and $B$ are sensitive variables and $Y$ is an outcome.}
%     \label{fig:interaction}
% \end{figure}
% \end{minipage}

















==> tex-input-files/text-interactionBias.tex <==

% \csam{As discussed, Interaction can be seen as a component of the correct quantity of $StatDisp$. So this section can be considered as decomposing $StatDisp$ with interaction term. So we need to define interaction as a bias in estimating $StatDisp$. That is, using this idea whenever we define interaction bias "If you estimate discrimination using formula x, your estimation is biased because of interaction bias". }

Interaction bias takes  place in the presence of two sensitive attributes when the value of one sensitive attribute influences the effect of the other sensitive attribute on the outcome (Figure~\ref{fig:interaction}). 

%Interaction bias is graphically illustrated in Figure~\ref{fig:interaction}. Note that regular DAGs are not able to express interaction. For this reason, we are employing the graphical representation proposed by \cite{weinberg2007can}. The arrows pointing to arrows, instead of nodes account for the interaction term. In a binary model interaction bias coincides with interaction term ($Interaction$) in the case of an intersectional sensitive attribute. Interaction bias also affects the individual measurement of the effect of sensitive attribute $A$ or $B$. 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=4cm]{figures/Interaction.pdf}
%     \caption{Interaction Bias, where $A$ and $B$ are sensitive variables and $Y$ is an outcome.}
%     \label{fig:interaction}
% \end{figure}



%\subsubsection{Binary model, Intersectional Sensitive Variable}





\begin{theorem}
\label{int_binary_A}
Under the assumption of no confounders between $A$ and $Y$ on one hand, and between $B$ and $Y$ on the other hand, adding up the single effects of $A$ and $B$ on $Y$ to estimate the discrimination due to both sensitive variables leads to a biased estimation. The amount of the bias ($IntBias$) coincides with the interaction term as follows:
%is not the same as adding up $StatDisp(Y,A)$ and $StatDisp(Y,B)$. In the presence of interaction, the measurement of bias against $A=0$ and $B=0$ with the sum of individual statistical disparity metrics would be biased:
\begin{align}
\intBias(Y,A,B)  &  =  Interaction(A,B)  \nonumber \\
& = P(y_1|a_1, b_1) - P(y_1|a_0, b_1) - P(y_1|a_1, b_0) + P(y_1|a_0, b_0)
\end{align}
\end{theorem}
%The bias here corresponds to the term $Interaction(A,B)$. 
\begin{theorem}
\label{th:interbin-2var}
Under the assumption of no confounders between $A$ and $Y$ on one hand, and between $B$ and $Y$ on the other hand, the interaction bias when estimating discrimination with respect to only $A$ is equal to:
\begin{align} \displaystyle
 \intBias(Y,A) & =P(b_1)Interaction(A,B)
\label{eq:inbiasA}
\end{align}
\end{theorem}
$\intBias(Y,B)$ is defined similarly as $P(a_1)Interaction(A,B)$.
For the linear model case, consider the true model:
\begin{equation}
\label{eq:linear-interaction}
Y = \beta_0 +\beta_1A + \beta_2B +\beta_3AB %+ \beta_4C
\end{equation}
and a biased model, that does not include interaction term $\beta_3$:
\begin{equation}
\label{eq:linear-interaction}
Y = \beta^{'}_0 +\beta^{'}_1A + \beta^{'}_2B %+ \beta^{'}_4C 
\end{equation}
Where $A$ and $B$ are binary sensitive attributes and  % $C$ is a set of covariates and 
$Y$ is a continuous value outcome.
The change in Y due to $A$ is $\beta_1 + \beta_3B$ and, similarly the change in Y due to $B$ is $\beta_2 + \beta_3A$~\cite{keele_stevenson_2021}. In this case, a measure of effect of $A$ ($\beta^{'}_1$) or $B$ ($\beta^{'}_2$) without an interaction term would be inaccurate.
%Next we define the bias introduced by not accounting for the interaction between two sensitive attributes. 

%\subsubsection{Linear model, Intersectional Sensitive Variable}

\begin{theorem}
\label{int_linear_AB}
Let $A$,$B$ and $Y$ be variables with linear regression coefficients as in Equation~\ref{eq:linear-interaction}. In a linear model with binary $A$ and $B$ the bias due to interaction, when measuring the discrimination with respect to both $A$ and $B$ is equal to:
\begin{align}
\intBias(Y,A,B) &= (\beta^{'}_1+\beta^{'}_2) -(\beta_1 + \beta_2 +\beta_3)= \beta_3\nonumber 
\end{align}
\end{theorem}
Intuitively, $\beta_3$ is part of an effect of the intersectional sensitive variable $A_1B_1$ on $Y$ that is left out of the estimation when fitting linear regression without the interaction term.

%\subsubsection{Linear model, Individual Sensitive Variable}
% The difference of measurement of effect of $A$ on $Y$ with interaction term ($\beta^{'}_1$) and without interaction term ($\beta_1$ ) depends on the value of $B$.

% \begin{equation}
% \beta^{'}_1 = \beta_1 +\beta_3 \label{notequal}
% \end{equation}
% when $B=1$, and
% \begin{equation}
% \beta^{'}_1 = \beta_1 \label{equal}
% \end{equation}
% when $B=0$.


\begin{theorem}
\label{IntBias(Y,A)avg}

Let $A$,$B$ and $Y$ be variables with linear regression coefficients as in Equation~\ref{eq:linear-interaction}. In a linear model with binary $A$ and $B$ the bias due to interaction, when measuring the discrimination with respect to only $A$ is equal to:
\begin{align}
\intBias(Y,A) &=  \beta_3\pr(B_1) 
\end{align}
\end{theorem}
Intuitively, $\intBias(Y,A)$ measures how wrong is the evaluation of effect of $A=1$ on average, for cases where $B=1$ or $B=0$. Similarly, $\intBias(Y,B) =  \beta_3\pr(A_1). $
% Note that the $IntBias(Y,A)$ is dependent on $\beta_3$ and the probability of $B=1$ (and, similarly, 
% $IntBias(B,A)$ is dependent on $\beta_3$ and the probability of $A=1$). 


% \csam{Let's discuss this sub-section (interaction bias, linear) in our next meeting.}


% \section{Experiments}

% The causal experiments on the real data are limited by the availability of true causal graphs for the benchmark fairness datasets. Furthemore, \cite{binkyte2022causal} show, that obtaining reliable causal graph with causal discovery algorithms is a complicated task. However, we will assume graphs existing in the literature to be the true graph for a given real dataset~\cite{zhang2018causal, huan2020fairness}. Although we cannot claim  the causal structure, that we use for the experiments is the ground truth, it is useful for experimentally demonstrating the behavior of causal biases. 
% In addition, the considered causal structure shows the presence of multiple causal biases at once. However, for the purposes of illustration, we control for a single type of bias separately. Namely, we measure a difference between statistical disparity and an effect when controlling for a particular type of bias, but not a causal effect, as causal effect would require to control for all the biases present in the data simultaneously. 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/confounderbias.png}
%     \caption{Confounder bias.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/confounderbias_withMult.png}
%     \caption{Confounder bias when controlling for all the confounders simultaniously.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/colliderbias.png}
%     \caption{Collider bias.}
%     \label{fig:interaction}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/interactionAandB.png}
%     \caption{Interaction bias A and B.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/interactionA.png}
%     \caption{Interaction bias A.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/3D_interactionbiases.png}
%     \caption{Interaction biases in linear model. Synthetic data.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/AB)_interaction_surface_plot.png}
%     \caption{Interaction bias A and B surface plot. Synthetic data.}
%     \label{fig:interaction}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/A_avginteractionbias_surface_plot.png}
%     \caption{Interaction bias A and B surface plot. Synthetic data.}
%     \label{fig:interaction}
% \end{figure}



% \begin{figure}[H]
%     \centering
%     \includegraphics[width=8cm]{figures/Ruta_Graphs/pairplot_interactionbiases.png}
%     \caption{Interaction biases in linear model pairplots. Synthetic data.}
%     \label{fig:interaction}
% \end{figure}







==> tex-input-files/text-measurementBias.tex <==

Measurement bias arises from how particular variable(s) are measured. A common example is when the ideal variable for a model is not measurable/observable and instead we rely on a proxy variable which behaves differently in different groups.
Figure~\ref{fig:measBias} shows a simple scenario when measuring accurately the discrimination based on $A$ requires adjusting on variable $Z$. However, if $Z$ is not measurable but a proxy variable $T$ is measurable, measurement bias occurs when we adjust on $T$ instead of $Z$.

% \begin{figure}[htp!]  
% \centering 
%   \begin{subfigure}[b]{0.4\linewidth}
%   {\includegraphics[scale=0.6]{./figures/measurementBias.pdf}}
% 	\caption{}
% 	\label{fig:measBiasa}
%  \end{subfigure}
%  \hspace{0.05\linewidth}
%  \begin{subfigure}[b]{0.4\linewidth}
%   {\includegraphics[scale=0.6]{./figures/measurementBiasLin.pdf}}
% 	\caption{}
% 	\label{fig:measBiasb}
%  \end{subfigure}
%  \caption{Measurement bias structure}
%  \end{figure}

% \begin{figure}[h]
% \centering
%   \includegraphics[scale=0.6]{./figures/measurementBiasLin.pdf}
% 	\caption{Simple measurement bias structure}
% 	\label{fig:measBias}
% \end{figure}
 



%\subsubsection{Binary model}



\begin{theorem} \label{th:measBin}
Assuming $A$, $Y$, and $Z$ binary variables such that $Z$ is not measurable, but only the error mechanism ($\pr(T|Z)$) is available, and that $\pr(a_0) = \pr(a_1) = \frac{1}{2}$, the difference in discrimination due to measurement bias, $\measBias(Y,A)$ can be expressed in terms of $\pr(T|Z)$ as follows:
\begin{align}
& \epsilon(\delta - \beta) + (1-\epsilon)(\gamma - \alpha) \nonumber \\
&\quad - \epsilon\big(\delta - \beta + 4\pr(t_1|z_0)(\beta - \delta + \gamma\Phi + \gamma\Psi)\big)\;Q \nonumber \\
&\quad - (1-\epsilon)\big(\gamma - \alpha + 4\pr(t_0|z_1)(\alpha - \gamma + \delta + \delta\Psi^{-1} + \beta\Phi^{-1})\big)\;R \label{eq:measBin}
\end{align}
where: 

% \begin{tabular}{ll}
% \begin{align}
% \epsilon &= \pr(t_1) \nonumber \\
% \tau &= \pr(t_0|a_0) \nonumber \\
% \alpha &= \pr(y_1|a_0,t_0) \nonumber \\
% \beta &= \pr(y_1|a_0,t_1) \nonumber \\
% \gamma &= \pr(y_1|a_1,t_0) \nonumber \\
% \delta &= \pr(y_1|a_1,t_1) \nonumber 
% \end{align}
% \begin{align}
% \Phi &= \frac{\epsilon + \frac{\tau}{2}-1}{\epsilon + \frac{\tau}{2}-\frac{1}{2}} \nonumber \\
% \Psi &= \frac{1 - \tau}{\tau} \nonumber \\
% Q &= \frac{1-\frac{\pr(t_0|z_1)}{\epsilon}}{1-\frac{\pr(t_0|z_1)}{2\epsilon}} \nonumber \\
% R &= \frac{1-\frac{\pr(t_1|z_0)}{1-\epsilon}}{1-\frac{\pr(t_1|z_0)}{2-2\epsilon}}
% \end{align}
% \end{tabular}

% \begin{array}{ll}
% \epsilon = \pr(t_1) & \displaystyle \Phi = \frac{\epsilon + \frac{\tau}{2}-1}{\epsilon + \frac{\tau}{2}-\frac{1}{2}} \\
% \tau = \pr(t_0|a_0) & \displaystyle  \Psi = \frac{1 - \tau}{\tau} \\
% \alpha = \pr(y_1|a_0,t_0) & \displaystyle  Q = \frac{1-\frac{\pr(t_0|z_1)}{\epsilon}}{1-\frac{\pr(t_0|z_1)}{2\epsilon}} \\
% \beta = \pr(y_1|a_0,t_1) & \displaystyle  R = \frac{1-\frac{\pr(t_1|z_0)}{1-\epsilon}}{1-\frac{\pr(t_1|z_0)}{2-2\epsilon}} \\
% \gamma = \pr(y_1|a_1,t_0)  \\
% \delta = \pr(y_1|a_1,t_1) 
% \end{array}

$\begin{array}{lllll}
\alpha = \pr(y_1|a_0,t_0) &  \gamma = \pr(y_1|a_1,t_0) & \displaystyle  Q = \frac{1-\frac{\pr(t_0|z_1)}{\epsilon}}{1-\frac{\pr(t_0|z_1)}{2\epsilon}} & \displaystyle \Phi = \frac{\epsilon + \frac{\tau}{2}-1}{\epsilon + \frac{\tau}{2}-\frac{1}{2}} & \epsilon = \pr(t_1)   \\
\beta = \pr(y_1|a_0,t_1) & \delta = \pr(y_1|a_1,t_1) & \displaystyle  R = \frac{1-\frac{\pr(t_1|z_0)}{1-\epsilon}}{1-\frac{\pr(t_1|z_0)}{2-2\epsilon}} & \displaystyle  \Psi = \frac{1 - \tau}{\tau} & \tau = \pr(t_0|a_0)
\end{array}$

% $\begin{array}{lll}
% \alpha = \pr(y_1|a_0,t_0) & \displaystyle  Q = \frac{1-\frac{\pr(t_0|z_1)}{\epsilon}}{1-\frac{\pr(t_0|z_1)}{2\epsilon}} & \epsilon = \pr(t_1)   \\
% \beta = \pr(y_1|a_0,t_1) & \displaystyle  R = \frac{1-\frac{\pr(t_1|z_0)}{1-\epsilon}}{1-\frac{\pr(t_1|z_0)}{2-2\epsilon}} & \tau = \pr(t_0|a_0) \\
%  \gamma = \pr(y_1|a_1,t_0) & \displaystyle \Phi = \frac{\epsilon + \frac{\tau}{2}-1}{\epsilon + \frac{\tau}{2}-\frac{1}{2}} & \\
% \delta = \pr(y_1|a_1,t_1)  & \displaystyle  \Psi = \frac{1 - \tau}{\tau} & 
% \end{array}$
\end{theorem}



% \begin{equation}
% ACE(Y,A) = \pr(y_1|do(a_1))_T - \pr(y_1|do(a_0))_Z \label{eq:measBias}
% \end{equation}
% where:
% \begin{align}
% &\pr(y_1|do(a))_Z = \nonumber \\
% & \frac{\pr(y_1,a,t_1)}{\pr(a|t_1)} \frac{\left(1-\frac{\pr(t_1|z_0)}{\pr(t_1|a,y_1)} \right)\left(1-\frac{\pr(t_1|z_0)}{\pr(t_1)} \right)}{1-\pr(t_1|z_0) \frac{\pr(a)}{\pr(t_1)}} \nonumber \\
% & + \frac{\pr(y_1,a,t_0)}{\pr(a|t_0)} \frac{\left(1-\frac{\pr(t_0|z_1)}{\pr(t_0|a,y_1)} \right)\left(1-\frac{\pr(t_0|z_1)}{\pr(t_0)} \right)}{1-\pr(t_0|z_1) \frac{\pr(a)}{\pr(t_0)}}
% \end{align}
% \end{theorem}

% % \begin{theorem}
% % Assuming that $Z$ is not measurable, but only the error mechanism ($\pr(T|Z)$) is available, $ACE(Y,A)$ can be expressed in terms of $\pr(T|Z)$ as follows:
% % \begin{equation}
% % ACE(Y,A) = \pr(y_1|do(a_1))_Z - \pr(y_1|do(a_0))_Z \label{eq:measBias}
% % \end{equation}
% % where:
% % \begin{align}
% % &\pr(y_1|do(a))_Z = \nonumber \\
% % & \frac{\pr(y_1,a,t_1)}{\pr(a|t_1)} \frac{\left(1-\frac{\pr(t_1|z_0)}{\pr(t_1|a,y_1)} \right)\left(1-\frac{\pr(t_1|z_0)}{\pr(t_1)} \right)}{1-\pr(t_1|z_0) \frac{\pr(a)}{\pr(t_1)}} \nonumber \\
% % & + \frac{\pr(y_1,a,t_0)}{\pr(a|t_0)} \frac{\left(1-\frac{\pr(t_0|z_1)}{\pr(t_0|a,y_1)} \right)\left(1-\frac{\pr(t_0|z_1)}{\pr(t_0)} \right)}{1-\pr(t_0|z_1) \frac{\pr(a)}{\pr(t_0)}}
% % \end{align}
% % \end{theorem}





% \subsubsection{Linear Model Case}



\begin{theorem}
Let $A$, $Y$, $Z$, and $T$ variables with linear regressions coefficients as in Figure~\ref{fig:measBias} which represents the basic measurement bias structure. Bias due to measurement error is equal to:
\begin{equation}
\measBias(Y,A) = \frac{{\sigma_z}^2 \beta \gamma ({\sigma_t}^2 - {\sigma_z}^2 \lambda^2)}{{\sigma_a}^2 {\sigma_t}^2 - {\sigma_z}^4 \lambda^2 \beta^2} \label{eq:measBiasLin}
\end{equation}
\end{theorem}


\begin{corollary}
For standardized variables $A$, $Y$, $Z$, and $T$, measurement bias is equal to: 
\begin{equation}
\measBias(Y,A) = \frac{\beta \gamma (1 - \lambda^2)}{1 - \lambda^2 \beta^2}
\end{equation}
\end{corollary}



% \subsection{Bias Analysis}

% \begin{figure*}[h]
% 	\centering %\hspace{-1cm}
% 	%{\includegraphics[scale=0.6]{./figures/confounding3D.pdf}}
%         {\includegraphics[scale=0.55]{./figures/MeasurementBiasAll.pdf}}
%         % {\includegraphics[width=12cm,height=10cm]{./figures/ConfoundingBias3D.pdf}}
% 	\caption{Measurement bias.}
% 	\label{fig:measAll}
% \end{figure*}





% \section{Interaction Bias and Effect Modification in the presence of more than one sensitive attribute}
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/InteractionBias-1.pdf}
%     \caption{Typed of Effect Modification and Interaction Biases}
%     \label{fig:enter-label}
% \end{figure}

% \begin{align}
% MeasBias(Y,A) & = ACE(Y,A)_{T} - ACE(Y,A) \nonumber \\
% & = \beta_{ya.t} - \beta_{ya.z} \nonumber \\
% & = \frac{{\sigma_z}^2 \beta \gamma ({\sigma_t}^2 - {\sigma_z}^2 \lambda^2)}{{\sigma_a}^2 {\sigma_t}^2 - {\sigma_z}^4 \lambda^2 \beta^2} \nonumber
% \end{align}



==> tex-input-files/text-selectionBias.tex <==

Selection bias occurs when there is collider variable caused by both the sensitive attribute $A$ and the outcome variable $Y$ and the data generation process implicitly conditions on that collider variable. The simplest case is illustrated in Figure~\ref{fig:simpleColl}. Consistent with previous work, a box around a variable indicates that data is generated by conditioning on that variable.  

% \begin{figure}[htp!]  
% \centering 
%   \begin{subfigure}[b]{0.4\linewidth}
%   {\includegraphics[scale=0.6]{./figures/simpleCollider.pdf}}
% 	\caption{}
% 	\label{fig:simpleColla}
%  \end{subfigure}
%  \hspace{0.05\linewidth}
%  \begin{subfigure}[b]{0.4\linewidth}
%   {\includegraphics[scale=0.6]{./figures/simpleColliderLinear.pdf}}
% 	\caption{}
% 	\label{fig:simpleCollb}
%  \end{subfigure}
%  \caption{Simple collider structure}
%  \end{figure}

%  \begin{figure}[h]  
% \centering 
%   \includegraphics[scale=0.6]{./figures/simpleColliderLinear.pdf}
% 	\caption{Simple collider structure}
% 	\label{fig:simpleColl}
%  \end{figure}



%\subsection{Binary Model}



\begin{theorem} \label{th:selBin}
Assuming $A$, $Y$, and $W$ binary variables and that $\pr(a_0) = \pr(a_1) = \frac{1}{2}$, the difference in discrimination due to collider structure is equal to:
\begin{align}
\selBias(Y,A) &= (1- \pr(w_0|a_0) - \pr(w_1))(-\alpha +\beta -\gamma + \delta) \label{eq:selBiasBin}
\end{align}
% where $\alpha, \beta, \gamma, \delta$ denote, respectively, 
% $\pr(y_1|x_0,z_0), \pr(y_1|x_0,z_1), \pr(y_1|x_1,z_0),\pr(y_1|x_1,z_1)$.
% \end{itemize}
 where, $\alpha = \pr(y_1|a_0,w_0)$, $\beta = \pr(y_1|a_0,w_1)$, $\gamma = \pr(y_1|a_1,w_0)$, and $\delta = \pr(y_1|a_1,w_1).$
% \begin{align}
% % % \tau &= P(x_0|z_0) \nonumber \\
% % % \epsilon &= P(z_0) \nonumber \\
% \alpha &= P(y_1|a_0,w_0) \nonumber \\
% \beta &= P(y_1|a_0,w_1) \nonumber \\
% \gamma &= P(y_1|a_1,w_0) \nonumber \\
% \delta &= P(y_1|a_1,w_1) \nonumber 
%  \end{align}   
\end{theorem}



%\subsection{Linear Model Case}

\begin{theorem} \label{th:selLin}
Let $A$, $Y$, and $Z$ variables with linear regressions coefficients as in Figure~\ref{fig:simpleColl} which represents the basic collider structure. Bias due to selection is equal to:
\begin{equation}
\displaystyle \selBias(Y,A) = \frac{\frac{\sigma_{ya}}{\sigma_a^2}\sigma_{wa}^2 - \sigma_{wa}\sigma_{yw}}{\sigma_a^2\sigma_w^2 - \sigma_{wa}^2} \label{eq:selLin1}
\end{equation}
Selection bias can also be expressed in terms of the linear regression coefficients as follows:
\begin{equation}
\selBias(Y,A) = \epsilon\;\;\frac{\sigma_a^4\alpha^2\eta + \sigma_a^4\alpha^3\epsilon - \sigma_y^2\sigma_a^2\eta -\sigma_y^2\sigma_a^2\alpha\epsilon}{\sigma_a^2\sigma_w^2 - (\sigma_a^2\eta + \sigma_a^2\alpha\epsilon)^2} \label{eq:selBiasLin}
\end{equation}
\end{theorem}



\begin{corollary}
For standardized variables $A$, $Y$, and $W$, selection bias can be expressed in terms of convariances as:
\begin{equation}
\displaystyle \selBias(Y,A) = \frac{\sigma_{ya}\sigma_{wa}^2 - \sigma_{wa}\sigma_{yw}}{1 - \sigma_{wa}^2}  \label{eq:selLin3}
\end{equation} 
And in terms of regression coefficient:
\begin{equation} 
\selBias(Y,A) = \epsilon \;\;\frac{\alpha^2\eta + \alpha^3\epsilon - \eta -\alpha\epsilon}{1 - (\eta + \alpha\epsilon)^2} \label{eq:selLin4}
\end{equation}
\end{corollary}
Equations~(\ref{eq:selLin3}) and~(\ref{eq:selLin4}) can be obtained from Equations~(\ref{eq:selLin1}) and~(\ref{eq:selBiasLin}) as $\sigma_a = \sigma_w = \sigma_y = 1$.

% \subsection{Bias Analysis}

% \begin{figure*}[h]
% 	\centering %\hspace{-1cm}
% 	%{\includegraphics[scale=0.6]{./figures/confounding3D.pdf}}
%         {\includegraphics[scale=0.55]{./figures/ColliderBiasAll.pdf}}
%         % {\includegraphics[width=12cm,height=10cm]{./figures/ConfoundingBias3D.pdf}}
% 	\caption{Selection bias.}
% 	\label{fig:collAll}
% \end{figure*}

% \begin{cor}
% Let $A$, $Y$, and $Z$ variables with linear regressions coefficients as in Figure~\ref{fig:simpleCollb} which represents the basic collider structure. Bias due to selection is equal to:
% \begin{equation}
% \displaystyle SelBias(Y,A) = \frac{\frac{\sigma_{ya}}{\sigma_a^2}\sigma_{wa}^2 - \sigma_{wa}\sigma_{yw}}{\sigma_a^2\sigma_w^2 - \sigma_{wa}^2} \label{eq:selLin1}
% \end{equation}
% Selection bias can also be expressed in terms of the linear regression coefficients as follows:
% \begin{equation}
% SelBias(Y,A) = \epsilon\;\;\frac{\sigma_a^4\alpha^2\eta + \sigma_a^4\alpha^3\epsilon - \sigma_y^2\sigma_a^2\eta -\sigma_y^2\sigma_a^2\alpha\epsilon}{\sigma_a^2\sigma_w^2 - (\sigma_a^2\eta + \sigma_a^2\alpha\epsilon)^2} \label{eq:selBiasLin}
% \end{equation}
% \end{theorem}

% For standardized variables $A$, $Y$, and $Z$, selection bias is~\cite{pearl2013linear}:
% \begin{equation}
% SelBias(Y,A) = \epsilon \frac{\alpha^2 \eta + \alpha^3 \epsilon - \eta - \alpha \epsilon }{1 - (\eta + \alpha\epsilon)^2}
% \end{equation}
% This is easily obtained from Eq.~\ref{eq:selBiasLin} as $\sigma_z = \sigma_a = \sigma_a = 1$.


